(In)approximability of Maximum Minimal FVS

We study the approximability of the NP-complete \textsc{Maximum Minimal Feedback Vertex Set} problem. Informally, this natural problem seems to lie in an intermediate space between two more well-studied problems of this type: \textsc{Maximum Minimal Vertex Cover}, for which the best achievable approximation ratio is $\sqrt{n}$, and \textsc{Upper Dominating Set}, which does not admit any $n^{1-\epsilon}$ approximation. We confirm and quantify this intuition by showing the first non-trivial polynomial time approximation for \textsc{Max Min FVS} with a ratio of $O(n^{2/3})$, as well as a matching hardness of approximation bound of $n^{2/3-\epsilon}$, improving the previous known hardness of $n^{1/2-\epsilon}$. The approximation algorithm also gives a cubic kernel when parameterized by the solution size. Along the way, we also obtain an $O(\Delta)$-approximation and show that this is asymptotically best possible, and we improve the bound for which the problem is NP-hard from $\Delta\ge 9$ to $\Delta\ge 6$. Having settled the problem's approximability in polynomial time, we move to the context of super-polynomial time. We devise a generalization of our approximation algorithm which, for any desired approximation ratio $r$, produces an $r$-approximate solution in time $n^{O(n/r^{3/2})}$. This time-approximation trade-off is essentially tight: we show that under the ETH, for any ratio $r$ and $\epsilon>0$, no algorithm can $r$-approximate this problem in time $n^{O((n/r^{3/2})^{1-\epsilon})}$, hence we precisely characterize the approximability of the problem for the whole spectrum between polynomial and sub-exponential time, up to an arbitrarily small constant in the second exponent.

==> NPhard.tex <==
\subsection{NP-hardness for $\Delta=6$}\label{sec:NP}

\begin{theorem}\label{thm:NP-h}
\textsc{Max Min FVS} is NP-hard on planar bipartite graphs with $\Delta=6$.
\end{theorem}

\begin{proof} We give a reduction from \textsc{Max Min VC},
which is NP-hard on planar bipartite graphs of maximum degree 3 \cite{ZZ1995}.
Note that the NP-hardness in \cite{ZZ1995} is stated for \textsc{Minimum
Independent Dominating Set}, but any independent dominating set is also a
maximal independent set (and vice-versa) and the complement of the minimum
maximal independent set of any graph is a maximum minimal vertex cover. Thus,
we also obtain NP-hardness for \textsc{Max Min VC} on the same instances.

We are given a graph $G=(V,E)$.  For each edge $e=(u,v)\in E$, we add a path of
length three from $u$ to $v$ going through two new vertices $e^{(1)},e^{(2)}$
(see Figure \ref{fig_core_K6}).  Note that $u,e^{(1)},e^{(2)},v$ form a cycle
of length 4.  Then we add two cycles of length 4,
$e^{(i)},c^{(i)}_{e1},c^{(i)}_{e2},c^{(i)}_{e3}$ and
$e^{(i)},c^{(i)}_{e4},c^{(i)}_{e5},c^{(i)}_{e6}$  for $i\in \{1,2\}$.  Let
$G'=(V',E')$ be the constructed graph.  Because  $\Delta(G)=3$, we have
$\Delta(G')=6$.  Moreover, since $G$ is planar and bipartite, $G'$ is also
planar and bipartite.  We will show that there is a minimal vertex cover of
size at least $k$ in $G$ if and only if there is a minimal feedback vertex set
of size at least $k+4|E|$ in $G'$.


\begin{figure}[tbp]
    \centering
    \includegraphics[width=8cm]{NP-hard.pdf}
    \caption{The edge gadget of $e=(u,v)$ in the constructed graph $G$.}
    \label{fig_core_K6}
\end{figure}



Given a minimal vertex cover $S$ of size at least $k$ in $G$, we construct the
set $S'=S\cup \bigcup_{e\in E}
\{c_{e1}^{(1)},c_{e4}^{(1)},c_{e1}^{(2)},c_{e4}^{(2)}\}$.  Then $|S'|\ge
k+4|E|$. Let us first argue that $S'$ is an fvs of $G'$. For each $e=(u,v)\in
E$ we have at least one of $u,v\in S$, without loss of generality let $u\in S$.
Now in $G'[V'\setminus S']$ the edges $(e^{(1)},e^{(2)})$ and $(e^{(2)},v)$ are
bridges and therefore cannot be part of any cycle. The remaining cycles going
through $e^{(1)},e^{(2)}$ are handled by
$\{c_{e1}^{(1)},c_{e4}^{(1)},c_{e1}^{(2)},c_{e4}^{(2)}\}$.  Furthermore, since
$G'[V\setminus S]$ is an independent set, it is also acyclic. To see that $S'$
is a minimal fvs, we remark that for each $c_{e1}^{(i)},c_{e4}^{(i)}$ contained
in $S'$ there is a private cycle in $G'[V'\setminus S']$. We also note that
since $S$ is a minimal vertex cover of $G$, for each $u\in S$, there exists
$v\not\in S$ with $e=(u,v)\in E$. This means that $u$ has the private cycle
formed by $\{u,v,e^{(1)},e^{(2)}\}$ in $G'[V'\setminus S']$.  Therefore, $S'$
is a minimal fvs.

Conversely, suppose we are given a minimal fvs $S'$ of $G'$ with $|S'|\ge
k+4|E|$.  We will edit $S'$ so that is contains only vertices in $V'\setminus
\bigcup_{e\in E}\{e^{(1)},e^{(2)}\}$, without decreasing its size. 

First, suppose $e^{(1)},e^{(2)}\in S'$, for some $e\in E$. We construct a new
minimal fvs $S''=S'\setminus\{e^{(2)}\}\cup\{c_{e1}^{(2)}, c_{e4}^{(2)}\}$
which is larger that $S'$, since by minimality we have $c_{ei}^{(2)}\not\in S'$
for $i\in\{1,\ldots,6\}$.  It is not hard to see that $S''$ is indeed an fvs,
as no cycle can go through $e^{(2)}$ in $G'[V'\setminus S'']$.  The two
vertices we added have a private cycle, while all vertices of $S'\cap S''$
retain their private cycles, so $S''$ is a minimal fvs. As a result in the
remainder we assume that $S'$ contains at most one of $\{e^{(1)}, e^{(2)}\}$
for all $e\in E$.

Suppose now that for some $e=(u,v)\in E$, we have $S'\cap\{u,v\}\neq\emptyset$
and $S'\cap\{e^{(1)},e^{(2)}\}\neq \emptyset$. Without loss of generality, let
$e^{(1)}\in S'$. We set
$S''=S'\setminus\{e^{(1)}\}\cup\{c_{e1}^{(1)},c_{e4}^{(1)}\}$ and claim that
$S''$ is a larger minimal fvs than $S$. Indeed, no cycle goes through $e^{(1)}$
in $G'[V'\setminus S'']$, the new vertices we added to $S'$ have private
cycles, and all vertices of $S'\cap S''$ retain their private cycles in
$G'[V'\setminus S'']$.  Therefore, we can now assume that if for some
$e=(u,v)\in E$ we have $S'\cap \{e^{(1)},e^{(2)}\}\neq \emptyset$ then
$u,v\not\in S'$.

For the remaining case, suppose that for some $e=(u,v)\in E$ we have
$u,v\not\in S'$ and (without loss of generality) $e^{(1)}\in S'$. We construct
the set $S''=S'\setminus\{e^{(1)}\}\cup\{c_{e1}^{(1)},c_{e4}^{(2)},u\}$. Note
that $|S''|\ge |S'|+2$. It is not hard to see that $S''$ is an fvs, since by
adding $c_{e1}^{(1)}, c_{e4}^{(1)}, v$ to our set we have hit all cycles
containing $e^{(1)}$ in $G'$. The problem now is that $S''$ is not necessarily
minimal. We greedily delete vertices from $S''$ to obtain a minimal fvs $S^*$.
We claim that in this process we cannot delete more than two vertices, that is
$|S^*\setminus S''|\le 2$.  To see this, we first note that
$c_{e1}^{(1)},c_{e4}^{(2)},u$ cannot be removed from $S''$ as they have private
cycles in $G[V'\setminus S'']$. Suppose now that $w_1\in S''\setminus S^*$ is
the first vertex we removed from $S''$, so $G'[(V'\setminus S'')\cup \{w_1\}]$
is acyclic.  This vertex must have had a private cycle in $G'[V'\setminus S']$,
which was necessarily going through $u$. Therefore, $G'[(V'\setminus S'')\cup
\{w_1\}]$ has a path connecting two neighbors of $u$ and this path does not
exist in $G'[(V'\setminus S'')]$. With a similar reasoning, removing another
vertex $w_2\in S''$ from the fvs will create a second path between neighbors of
$u$ in the induced forest. We conclude that this cannot happen a third time,
since $|N(u)|\le 3$, and if we create three paths between neighbors of $u$,
this will create a cycle. As a result, $|S^*|\ge |S'|$. We assume in the
remainder that $S'$ does not contain $e^{(1)},e^{(2)}$ for any $e\in E$.

Now, given a minimal fvs $S'$ of $G'$ with $|S'|\ge k+4|E|$ and $S'\cap
(\cup_{e\in E} \{e^{(1)},e^{(2)}\}) = \emptyset$ we set $S=S'\cap V$ and claim
that $S$ is a minimal vertex cover of $G$ with $|S|\ge k$. Indeed $S$ is a
vertex cover, as for each $e=(u,v)\in E$, if $u,v\not\in S'$ then we would get
the cycle formed by $\{u,v,e^{(1)},e^{(2)}\}$. To see that $S$ is minimal,
suppose $N_G[u]\subseteq S'$. We claim that in that case $u$ has no private
cycle in $G'[V'\setminus S']$ (this can be seen by deleting all bridges in
$G'[V'\setminus S']$, which leaves $u$ isolated). This contradicts the
minimality of $S'$ as an fvs of $G'$. Finally, we argue that $|S'\setminus
V|\le 4|E|$, which gives the desired bound on $|S|$. Consider an $e=(u,v)\in
E$. $S'$ cannot contain more than one vertex among
$c_{e1}^{(1)},c_{e2}^{(1)},c_{e3}^{(1)}$, since any of these vertices hits the
cycle that goes through the others. With similar reasoning for the three other
length-four cycles we conclude that $S'$ contains at most $4$ vertices for each
edge $e\in E$.  \end{proof}



==> inapprox.tex <==
In this section we establish lower bound results showing that the approximation
algorithms given in Theorems \ref{thm:algpoly} and \ref{thm:subexp} are
essentially optimal, under standard complexity assumptions.

\subsection{Hardness of Approximation in Polynomial Time}

We begin by showing that the best approximation ratio achievable in polynomial
time is indeed (essentially) $n^{2/3}$. For this, we rely on the celebrated
result of H{\aa}stad on the hardness of approximating \textsc{Max Independent
Set}, which was later derandomized by Zuckerman, cited below.

\begin{theorem}\cite{Hastad99,Zuckerman07} For any $\epsilon>0$, there is no
polynomial time algorithm which approximates \textsc{Max Independent Set} with
a ratio of $n^{1-\epsilon}$, unless $\text{P}=\text{NP}$. \end{theorem}

Starting from this result, we present a reduction to \textsc{Max Min FVS}.

\begin{theorem}\label{thm:Inapprox} For any $\epsilon>0$, \textsc{Max Min 
FVS} is inapproximable within a factor of $n^{2/3-\epsilon}$ unless $\text{P}=\text{NP}$.
\end{theorem} 

\begin{proof} We give a gap-preserving reduction from \textsc{Max Independent
Set}, which cannot be approximated within a factor of $n^{1-\epsilon}$, unless
$\text{P}=\text{NP}$.  We are given a graph $G=(V,E)$ on $n$ vertices as an instance of
\textsc{Max Independent Set}. Recall that $\alpha(G)$ denotes the size of the
maximum independent set of $G$.

We transform $G$ into an instance of \textsc{Max Min FVS} as follows: For
every pair of $u,v\in V$, we add $n$ vertices such that they are adjacent only
to $u$ and $v$.  We denote by $I_{uv}$ the set of such vertices.  Then $I_{uv}$
is an independent set. Let $G'=(V',E')$ be the constructed graph. 

We now make the following two claims:

\begin{claim} $\mmfvs(G')\ge (n-1){\alpha(G)\choose 2}$ \end{claim} 

\begin{proof} We construct a minimal fvs of $G'$ as follows: let $C$ be a
minimum vertex cover of $G$. Then we begin with the set that contains $C$ and
the union of all $I_{uv}$ (which is clearly an fvs) and remove vertices from it
until it becomes minimal. Let $S$ be the final minimal fvs. We observe that for
all $u,v\in V\setminus C$, $S$ contains at least $n-1$ of the vertices of
$I_{uv}$. Since $C$ is a minimum vertex cover of $G$, there are
$\alpha(G)\choose 2$ pairs $u,v\in V\setminus C$. \end{proof}

\begin{claim} $\mmfvs(G')\le n{2\alpha(G)\choose 2}+n$ \end{claim}

\begin{proof} 

Let $S$ be a minimal fvs of $G'$ and $F$ be the corresponding forest. It
suffices to show that $|S\setminus V|\le n{2\alpha(G)\choose 2}$, since $|S\cap
V|\le n$. Consider now a set $I_{uv}$. If $u\in S$ or $v\in S$, then
$I_{uv}\cap S=\emptyset$, because all vertices of $I_{uv}$ have at most one
neighbor in $F$, and are therefore redundant. So, $I_{uv}$ contains (at most
$n$) vertices of $S$ only if $u,v\in F$. However, $|F\cap V| \le 2 \alpha(G)$,
because $F$ is bipartite, so $F\cap V$ induces two independent sets, both of
which must be at most equal to the maximum independent set of $G$. So the
number of pairs $u,v\in F\cap V$ is at most $2\alpha(G)\choose 2$ and since
each corresponding $I_{uv}$ has size $n$, we get the promised bound.
\end{proof}

The two claims together imply that there exist constants $c_1,c_2$ such that
(for sufficiently large $n$) we have $c_1n(\alpha(G))^2 \le \mmfvs(G') \le
c_2n(\alpha(G))^2$. That is, $\mmfvs(G') = \Theta(n(\alpha(G))^2)$.

Suppose now that there exists a polynomial-time approximation algorithm which,
given a graph $G'$, produces a minimal fvs $S$ with the property
$\frac{\mmfvs(G')}{r}\le|S|\le \mmfvs(G')$, that is, there exists an
$r$-approximation for \textsc{Max Min FVS}. Running this algorithm on the
instance we constructed, we obtain that $\frac{c_1n(\alpha(G))^2}{r} \le |S|
\le c_2n(\alpha(G))^2$. Therefore,   $\frac{\alpha(G)}{\sqrt{rc_2/c_1}} \le
\sqrt{\frac{|S|}{c_2n}} \le \alpha(G)$. As a result, we obtain an $O(\sqrt{r})$
approximation for the value of $\alpha(G)$. We therefore conclude that, unless
$\text{P}=\text{NP}$, any such algorithm must have $\sqrt{r}>n^{1-\epsilon}$, for any
$\epsilon>0$, hence, $r>n^{2-\epsilon}$, for any $\epsilon>0$. Since the graph
$G'$ has $N=\Theta(n^3)$ vertices, we get that no approximation algorithm can
achieve a ratio of $N^{2/3-\epsilon}$. \end{proof}

We notice that in the construction of the previous theorem, the maximum degree
of the graph is approximately equal to the approximation gap.  Thus, the
following corollary also holds.

\begin{corollary}\label{cor:inapprox_deg} For any positive constant $\epsilon$,
\textsc{Max Min FVS} is inapproximable within a factor of
$\Delta^{1-\epsilon}$ unless $\text{P}=\text{NP}$.  \end{corollary}

\subsection{Hardness of Approximation in Sub-Exponential Time}

In this section we extend Theorem \ref{thm:Inapprox} to the realm of
sub-exponential time algorithms. We recall the following result of Chalermsook
et al.

\begin{theorem}\label{thm:chal}\cite{ChalermsookLN13} For any $\epsilon>0$
and any sufficiently large $r$, if there exists an $r$-approximation algorithm
for \textsc{Max Independent Set} running in $2^{(n/r)^{1-\epsilon}}$, then the
randomized ETH is false.  \end{theorem}

We remark that Theorem \ref{thm:chal}, which gives an almost tight running time
lower bound for \textsc{Max Independent Set}, has already been used as a
starting point to derive a similarly tight bound for the running time of any
sub-exponential time approximation for \textsc{Max Min VC}. Here,
we modify the proof of Theorem \ref{thm:Inapprox} to obtain a similarly tight
result for \textsc{Max Min FVS}. Nevertheless, the reduction for
\textsc{Max Min FVS} is significantly more challenging, because the ideas
used in Theorem \ref{thm:Inapprox} involve an inherent quadratic (in $n$)
blow-up of the size of the instance. As a result, in addition to executing an
appropriately modified version of the reduction of Theorem \ref{thm:Inapprox},
we are forced to add an extra ``sparsification'' step, and use a probabilistic
analysis with Chernoff bounds to argue that this step does not destroy the
inapproximability gap.

\begin{theorem}\label{thm:Inapprox2} For any $\epsilon>0$ and any sufficiently
large $r$, if there exists an $r$-approximation algorithm for \textsc{Max
Min FVS} running in $2^{(n/r^{3/2})^{1-\epsilon}}$, then the randomized ETH
is false.  \end{theorem}








==> intro.tex <==
\section{Introduction}\label{sec:intro}

In a graph $G=(V,E)$, a set $S\subseteq V$ is called a \emph{feedback vertex
set} (fvs for short) if the subgraph induced by $V\setminus S$ is a forest.
Typically, fvs is studied with a minimization objective: given a graph we are
interested in finding the best (that is, smallest) fvs.  In this paper we are
interested in an objective which is, in a sense, the inverse: we seek an fvs
$S$ which is as \emph{large} as possible, while still being minimal. We call
this problem \textsc{Max Min FVS}.

MaxMin and MinMax versions of many famous optimization problems have recently
attracted much interest in the literature (we give references below) and
\textsc{Max Min FVS} can be seen as a member of this framework.  Although the
initial motivation for studying such problems was a desire to analyze the worst
possible performance of a naive heuristic, these problems have gradually been
revealed to possess a rich combinatorial structure that makes them interesting
in their own right. Our goal in this paper is to show that \textsc{Max Min FVS}
displays an interesting complexity behavior with respect to its
approximability.

Our motivation for focusing on \textsc{Max Min FVS} is the contrast between two
of its more well-studied cousins: the \textsc{Max Min Vertex Cover} and
\textsc{Upper Dominating Set} problems, where the objective is to find the
largest minimal vertex cover or dominating set respectively. At first glance,
one would expect \textsc{Max Min VC} to be the easier of these two problems:
both problems can be seen as trying to find the largest minimal hitting set of
a hypergraph, but in the case of \textsc{Max Min VC} the hypergraph has a very
restricted structure, while in \textsc{UDS} the hypergraph is essentially
arbitrary. This intuition turns out to be correct: while \textsc{UDS} admits no
$n^{1-\epsilon}$-approximation \cite{Bazgan2018}, \textsc{Max Min VC} admits a
$\sqrt{n}$-approximation (but no $n^{1/2-\epsilon}$-approximation)
\cite{Boria2015}.

This background leads us to the natural question of the approximability of
\textsc{Max Min FVS}. Intuitively, one may be tempted to think that
this problem should be harder than \textsc{Max Min VC}, since hitting cycles is
more complex than hitting edges, but easier than \textsc{UDS}, since hitting
cycles still offers us more structure than an arbitrary hypergraph. However, to
the best of our knowledge, no $n^{1-\epsilon}$-approximation algorithm is
currently known for \textsc{Max Min FVS} (so the problem could be as hard as
\textsc{UDS}), and the best hardness of approximation bound known is
$n^{1/2-\epsilon}$ \cite{MishraS01} (so the problem could be as easy as \textsc{Max Min VC}).

Our main contribution in this paper is to fully answer this question, confirming and
precisely quantifying the intuition that \textsc{Max Min FVS} is a
problem that lies ``between'' \textsc{Max Min VC} and \textsc{UDS}: We give a
polynomial-time approximation algorithm with ratio $O(n^{2/3})$ and a hardness
of approximation reduction which shows that (unless $\text{P}=\text{NP}$) no polynomial-time
algorithm can obtain a ratio of $n^{2/3-\epsilon}$, for any $\epsilon>0$. This
completely settles the approximability of the problem in polynomial time. Along
the way, we also give an approximation algorithm with ratio $O(\Delta)$, show
that no algorithm can achieve ratio $\Delta^{1-\epsilon}$, for any
$\epsilon>0$, and improve the best known NP-completeness proof for \textsc{Max
Min FVS} from $\Delta\ge 9$ \cite{MishraS01} to $\Delta \ge 6$, where $\Delta$
is the maximum degree of the input graph.

One interesting aspect of our results is that they have an interpretation from
extremal combinatorics which nicely mirrors the situation for \textsc{Max Min
VC}. Recall that a corollary of the $\sqrt{n}$-approximation for \textsc{Max
Min VC} \cite{Boria2015} is that any graph without isolated vertices has a
minimal vertex cover of size at least $\sqrt{n}$, and this is tight (see Remark
\ref{rem:vc}). Hence, the algorithm only needs to trivially preprocess the
graph (deleting isolated vertices) and then find this set, which is guaranteed
to exist.  Our algorithms can be seen in a similar light: we prove that if one
applies two almost trivial pre-processing rules to a graph (deleting leaves and
contracting edges between degree-two vertices), a minimal fvs of size at least
$n^{1/3}$ (and $\Omega(n/\Delta)$) is always guaranteed to exist, and this is
tight (Corollary \ref{cor:extr} and Remark \ref{rem:fvs}).  Thus, the
approximation ratio of $n^{2/3}$ is automatically guaranteed for any graph
where we exhaustively apply these very simple rules and our algorithms only
have to work to construct the promised set. This makes it somewhat remarkable
that the ratio of $n^{2/3}$ turns out to be best possible.

Having settled the approximability of \textsc{Max Min FVS} in polynomial time,
we consider the question of how much time needs to be invested if one wishes to
guarantee an approximation ratio of $r$ (which may depend on $n$) where $r
<n^{2/3}$. This type of time-approximation trade-off was extensively studied by
Bonnet et al. \cite{Bonnet2018}, who showed that \textsc{Max Min Vertex Cover}
admits an $r$-approximation in time $2^{O(n/r^2)}$ and this is optimal under
the randomized ETH.

For \textsc{Max Min FVS} we cannot hope to obtain a trade-off with performance
exponential in $n/r^2$, as this implies a polynomial-time
$\sqrt{n}$-approximation. It therefore seems more natural to aim for a running
time exponential in $n/r^{3/2}$. Indeed, generalizing our polynomial-time
approximation algorithm, we show that we can achieve an $r$-approximation in
time $n^{O(n/r^{3/2})}$. Although this algorithm reuses some ingredients from
our polynomial-time approximation, it is significantly more involved, as it is
no longer sufficient to compare the size of our solution to $n$. We complement
our result with a lower bound showing that our algorithm is essentially best
possible under the randomized ETH for any $r$ (not just for polynomial time),
or more precisely that the exponent of the running time of our algorithm can
only be improved by $n^{o(1)}$ factors.

\subparagraph*{Related work} To the best of our knowledge, \textsc{Max Min FVS}
was first considered by Mishra and Sikdar \cite{MishraS01}, who showed that the
problem does not admit an $n^{1/2-\epsilon}$ approximation (unless $\text{P}=\text{NP}$), and
that it remains APX-hard for $\Delta\ge 9$. On the other hand, \textsc{UDS} and
\textsc{Max Min VC} are well-studied problems, both in the context of
approximation and in the context of parameterized complexity
\cite{AbouEishaHLMRZ18,Bazgan2018,Boria2015,BoyaciM17,ChestonFHJ90,CourcelleMR00,Demange1999,HenningP20,JacobsonP90,Zehavi2017,ZZ1995}.
Many other classical optimization problems have recently been studied in the
MaxMin or MinMax framework, such as \textsc{Max Min Separator}
\cite{Hanaka2019}, \textsc{Max Min Cut} \cite{EtoHKK2019}, \textsc{Min Max 
Knapsack} (also known as the \textsc{Lazy Bureaucrat Problem})
\cite{ArkinBMS03,Furini2017,GourvesMP13}, and \textsc{Max Min Edge Cover}
\cite{KhoshkhahGMS20,DBLP:conf/ttcs/HarutyunyanGMMP20}. Some problems in this area also arise naturally in other
forms and have been extensively studied, such as \textsc{Min Max Matching}
(also known as \textsc{Edge Dominating Set} \cite{IwaideN16}) and
\textsc{Grundy Coloring}, which can be seen as a Max Min version of
\textsc{Coloring} \cite{AboulkerB0S20,BelmonteKLMO20}.

The idea of designing super-polynomial time approximation algorithms which
obtain guarantees better than those possible in polynomial time has attracted
much attention in the last decade
\cite{BansalCLNN19,BourgeoisEP09,CyganKW09,CyganP10,EscoffierPT14,FotakisLP16,KatsikarelisLP19}.
As mentioned, the result closest to the time-approximation trade-off we give in
this paper is the approximation algorithm for \textsc{Max Min VC} given by
Bonnet et al. \cite{Bonnet2018}. It is important to note that such trade-offs
are only generally known to be tight up to poly-logarithmic factors in the
exponent of the running time. As explained in \cite{Bonnet2018}, current lower
bound techniques can rule out improvements in the running time that shave at
least $n^\epsilon$ from the exponent, but not improvements which shave
poly-logarithmic factors, due to the state of the art in quasi-linear PCP
constructions. Indeed, such improvements are sometimes possible
\cite{BansalCLNN19} and are conceivable for \textsc{Max Min VC} and \textsc{Max
Min FVS}. Lower bounds for this type of algorithm rely on the (randomized)
Exponential Time Hypothesis (ETH), which states that there is no (randomized)
algorithm for \textsc{3-SAT} running in time $2^{o(n)}$.



